An Inverse QSAR Method Based on Linear Regression and Integer Programming

Recently a novel framework has been proposed for designing the molecular structure of chemical compounds using both artificial neural networks (ANNs) and mixed integer linear programming (MILP). In the framework, we first define a feature vector $f(C)$ of a chemical graph $C$ and construct an ANN that maps $x=f(C)$ to a predicted value $\eta(x)$ of a chemical property $\pi$ to $C$. After this, we formulate an MILP that simulates the computation process of $f(C)$ from $C$ and that of $\eta(x)$ from $x$. Given a target value $y^*$ of the chemical property $\pi$, we infer a chemical graph $C^\dagger$ such that $\eta(f(C^\dagger))=y^*$ by solving the MILP. In this paper, we use linear regression to construct a prediction function $\eta$ instead of ANNs. For this, we derive an MILP formulation that simulates the computation process of a prediction function by linear regression. The results of computational experiments suggest our method can infer chemical graphs with around up to 50 non-hydrogen atoms.

==> Constraints_MILP_2LM_normalization.tex <==

   %%%\newpage%%%
\subsection{Constraints for Normalization  of Feature Vectors} 
% \subsection{Constraints for Normalization or Standardization of Feature Vectors}  
\label{sec:NSFV}%%%%%%%%%%%%%%%


  By introducing a tolerance $\varepsilon>0$   in the conversion 
 between integers and reals, we include the following constraints for 
normalizing of a  feature vector   $f(\C)=(x_1,x_2,\ldots,x_K)$: 
\begin{equation}\label{eq:normalization2}
\frac{(1 - \varepsilon)(x_i  - \min(\dcp_i;D_\pi))}
{ \max(\dcp_i;D_\pi) - \min(\dcp_i;D_\pi) }
\leq \widehat{ x}_i  \leq 
\frac{(1 + \varepsilon) ( x_i - \min(\dcp_i;D_\pi))}
{ \max(\dcp_i;D_\pi) - \min(\dcp_i;D_\pi) }, 
~ i\in [1,K].  
\end{equation} 
An example of  a tolerance is $\varepsilon=1\times 10^{-5}$.

% By introducing a tolerance $\varepsilon>0$   in the conversion 
% between integers and reals, we include the following constraints for 
% standardizing of a  feature vector   $f(G)=(x_1,x_2,\ldots,x_K)$: 
% \begin{equation}\label{eq:standardization2}
% \frac{(1 - \varepsilon)( x_i   - \avg(\dcp_i;D_\pi))}
% { \sd(\dcp_i;D_\pi) - \avg(\dcp_i;D_\pi) }
% \leq \widetilde{ x}_i  \leq 
%    \frac{ (1 + \varepsilon)(x_i  - \avg(\dcp_i;D_\pi))}
%    { \sd(\dcp_i;D_\pi) }, ~ i\in [1,K].  
%\end{equation} 
%An example of  a tolerance is $\varepsilon=0.01$.
 
  


